Mechanism Design for Efficient Nash Equilibrium in Oligopolistic Markets

This paper investigates the efficiency loss in social cost caused by strategic bidding behavior of individual participants in a supply-demand balancing market, and proposes a mechanism to fully recover equilibrium social optimum via subsidization and taxation. We characterize the competition among supply-side firms to meet given inelastic demand, with linear supply function bidding and the proposed efficiency recovery mechanism. We show that the Nash equilibrium of such a game exists under mild conditions, and more importantly, it achieves the underlying efficient supply dispatch and the market clearing price that reflects the truthful system marginal production cost. Further, the mechanism can be tuned to guarantee self-sufficiency, i.e., taxes collected counterbalance subsidies needed. Extensive numerical case studies are run to validate the equilibrium analysis, and we employ individual net profit and a modified version of Lerner index as two metrics to evaluate the impact of the mechanism on market outcomes by varying its tuning parameter and firm heterogeneity.

==> edits_pcyou.tex <==
\usepackage{ifthen}
\newboolean{showcomments}
\setboolean{showcomments}{true}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{todonotes}
\usepackage{soul}

\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}

%ADD CITES
\newcommand{\addcite}[0]{\ifthenelse{\boolean{showcomments}}
{\textcolor{purple}{(add cite(s)) }}{}}%

% Comments
\newcommand{\you}[1]{  \ifthenelse{\boolean{showcomments}}
{\todo[inline,color=bleudefrance]{PCY: #1}}{}}
% \newcommand{\youmargin2}[1]{\ifthenelse{\boolean{showcomments}}{\marginpar{\color{bleudefrance}\tiny PCY: #1}}{}}
\newcommand{\youmargin}[1]{  \ifthenelse{\boolean{showcomments}}
{\todo[color=bleudefrance,size=\tiny]{PCY: #1}} {}}

\makeatletter
\if@todonotes@disabled
\newcommand{\hlfix}[2]{\hl{#1}}
\else
\newcommand{\hlfix}[2]{\hl{#1}\todo[color=bleudefrance,size=\tiny]{PCY: #2}}
\fi
\makeatother


%\usepackage{comment}
%\newcommand{\slow}[1]{\ifthenelse{\boolean{showcomments}}
%	{ \textcolor{red}{(SL:  #1)}}{}}
\newcommand{\pcyou}[1]{\ifthenelse{\boolean{showcomments}}
	{ \textcolor{red}{(PCY:  #1)}}{}}
%\newcommand{\john}[1]{\ifthenelse{\boolean{showcomments}}
%	{ \textcolor{green}{(jp:  #1)}}{}}


%Edits to be highlighted
\newboolean{showedits}
\setboolean{showedits}{true}
\usepackage[xcolor=bleudefrance]{changes}
\definechangesauthor[color=bleudefrance]{PCY}
\newcommand{\ayou}[1]{
\ifthenelse{\boolean{showedits}}
{\added[id=PCY]{#1}}
{#1}
}
\newcommand{\chyou}[2]{
\ifthenelse{\boolean{showedits}}
{\replaced[id=PCY]{#1}{#2}}
{#1}
}
\newcommand{\dyou}[1]{
\ifthenelse{\boolean{showedits}}
{\deleted[id=PCY]{#1}}
{}
}
%\listoftodos[{\color{red}\textbf{List of comments/suggestions}}]


%\usepackage{epsfig, latexsym, times, bbm}
%\usepackage{color}
%\usepackage{colortbl}
%\usepackage{array}
%\usepackage{cite}
%\usepackage{amsmath}
%\usepackage{graphics}
%\usepackage{graphicx}
%\usepackage{amssymb}
%\usepackage{url}
%\usepackage{comment}
%%\usepackage{caption}
%\usepackage{multirow}
%\def\UrlBreaks{\do\/\do-}
%%\captionsetup{justification   = raggedright, singlelinecheck = false}
%\usepackage{bbding}
%\usepackage{amsfonts}
%\usepackage{cases}
%\usepackage{subfigure}
%%\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage{mathrsfs}
%\usepackage{bm}
%\usepackage{verbatim}
%\usepackage{enumerate}
%%\usepackage[colorlinks,
%%            linkcolor=black, % ref, red
%%            anchorcolor=black, % bookmark, blue
%%            citecolor=black % cite, green
%%            ]{hyperref}
%\usepackage{booktabs}
%\usepackage[linesnumbered,ruled,longend]{algorithm2e}
%\usepackage{textcomp}
%%% mac unsupported
%%\usepackage{slashbox}
%\usepackage{subeqnarray}
%
%
%
%
%
%
%
%
%%% added
%\def\ba{\begin{array}}
%	\def\ea{\end{array}}
%\newcommand{\beq}{\begin{equation}}
%	\newcommand{\eeq}{\end{equation}}
%\newcommand{\bq}{\begin{eqnarray}}
%	\newcommand{\eq}{\end{eqnarray}}
%\newcommand{\bqn}{\begin{eqnarray*}}
%	\newcommand{\eqn}{\end{eqnarray*}}
%\newcommand{\bee}{\begin{enumerate}}
%	\newcommand{\eee}{\end{enumerate}}
%\newcommand{\bi}{\begin{itemize}}
%	\newcommand{\ei}{\end{itemize}}
%\newcommand{\bseq}{\begin{subequations}}
%\newcommand{\eseq}{\end{subequations}}
%\newcommand{\qed}{\hfill{$\blacksquare$}}
%\newcommand{\ii}{\textbf{i}}
%\newcommand{\diag}{\textrm{diag}}
%\newcommand{\blockdiag}{\textrm{blockdiag}}
%
%\newtheorem{definition}{\textbf{Definition}}
%\newtheorem{proposition}{\textbf{Proposition}}
%\newtheorem{corollary}{\textbf{Corollary}}
%\newtheorem{lemma}{\textbf{Lemma}}
%\newtheorem{theorem}{\textbf{Theorem}}
%\newtheorem{remark}{\textbf{Remark}}
%
%
%
%\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
%\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}
%\newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{#1}}
%\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}
%\newcommand{\cell}[3]{\parbox[c][#2][c]{#1}{\makebox[#1]{#3}}}
%
%\renewcommand\thepage{}
%\renewcommand{\arraystretch}{1.3}
%
%% correct bad hyphenation here
%\hyphenation{op-tical net-works semi-conduc-tor}
%\allowdisplaybreaks


